CHOP: Integrating ChatGPT into EFL Oral Presentation Practice

English as a Foreign Language (EFL) students often struggle to deliver oral presentations due to a lack of reliable resources and the limited effectiveness of instructors' feedback. Large Language Model (LLM) can offer new possibilities to assist students' oral presentations with real-time feedback. This paper investigates how ChatGPT can be effectively integrated into EFL oral presentation practice to provide personalized feedback. We introduce a novel learning platform, CHOP (ChatGPT-based interactive platform for oral presentation practice), and evaluate its effectiveness with 13 EFL students. By collecting student-ChatGPT interaction data and expert assessments of the feedback quality, we identify the platform's strengths and weaknesses. We also analyze learners' perceptions and key design factors. Based on these insights, we suggest further development opportunities and design improvements for the education community.

==> sources/tables/ChatGPT_prompts.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{System prompt and feedback prompts used to guide ChatGPT}
\begin{tabular}{@{}cll@{}}
\toprule
\multicolumn{3}{c}{System prompt} \\ \midrule
\multicolumn{3}{l}{\begin{tabular}[c]{@{}l@{}}You are a presentation assistant for an EFL student.\\ \\ You will be given the user's presentation rehearsals, and you will provide feedback on them.\\ \\ The user is presenting at a <presentation location> in front of <target audience>.\\ \\ Here are the summarized contents of each slide of the presentation.\\ \\ \#\#\#Summarized slide contents: <Summarized slide contents>\end{tabular}} \\ \midrule
\multicolumn{3}{c}{Feedback prompt} \\ \midrule
\multicolumn{2}{c}{Grammar, Vocabulary, Content, Organzation} &
  \multicolumn{1}{c}{Delivery} \\ \midrule
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}The following is the transcript of a rehearsal from slide <start slide> to <end slide>:\\ \\ \#\#\#transcript: <transcript>\\ \\ Using the transcript, provide feedback on this rehearsal according to the following rubric:\\ \\ \#\#\#Presentation rubric: <presentation rubric>\\ \\ \#\#\#Feedback type: <feedback type>\\ \\ The final output should be in the following format:\\ \\\#\#\#Output example: <Output example>\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}The following is the transcript of a rehearsal from slide <start slide> to <end slide>:\\ \\ \#\#\#transcript: <transcript>\\ \\ The following are the assessment results of the delivery of the rehearsal:\\ \\\#\#\#Assessment results: <Delivery scores and brief explanation>\\ \\ The following are words that received low pronunciation scores:\\ \\\#\#\#Poor pronunciation words: <Words with low pronunciation scores>\\ \\ Provide clear, concise feedback on the delivery of this rehearsal.\\ \\ The final output should be in the following format:\\ \\\#\#\#Output example: <Output example>\end{tabular} \\ \bottomrule
\end{tabular}%
\label{tab:ChatGPT_prompts}
\end{table*}



==> sources/tables/FGI_questions.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l@{}}
\toprule
\multicolumn{1}{c}{Experience with Oral Presentations}                                                                    \\ \midrule
How did you prepare for your oral presentations?                                                                          \\
What do you think are the key elements that contribute to an effective oral presentation?                                 \\
What challenges did you encounter while preparing for and delivering oral presentations?                                  \\
How did you attempt to overcome these challenges?                                                                         \\ \midrule
\multicolumn{1}{c}{Feedback Preferences}                                                                                  \\ \midrule
Below are feedback samples with different styles: one is direct and the other is indirect. Which do you prefer and why?   \\
Below are feedback samples with different styles: one is positive and the other is negative. Which do you prefer and why? \\
Below are feedback samples with different styles: one is vague and the other is specific. Which do you prefer and why?    \\
Below are feedback samples with different styles: one is straightforward and the other is polite. Which do you prefer and why? \\
Below are feedback samples with different styles: one is immediate and the other is delayed. Which do you prefer and why? \\ \bottomrule
\end{tabular}%
}
\caption{Questions used in the focus group interview}
\label{tab:FGI_questions}
\end{table*}

==> sources/tables/post-survey_questions.tex <==
\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l@{}}
\toprule
\multicolumn{1}{c}{Student’s experience with the platform}        \\ \midrule
How effective was the feedback in the following areas: Vocabulary, Grammar, Content, Delivery, Organization? \\
How effective was the feedback during partial/full rehearsal?     \\
How reliable did you find the feedback?                           \\
How well did ChatGPT understand the content of your presentation? \\
What aspects did you like or dislike about the partial/full rehearsal feedback?                              \\
What was the feedback particularly helpful for?                   \\
What was the feedback particularly unhelpful for?                 \\ \midrule
\multicolumn{1}{c}{Potential learning effects}                    \\ \midrule
To what extent did the platform improve your confidence and reduce nervousness in presenting?                \\
To what extent did the platform help enhance your vocabulary?     \\
To what extent did the platform help you identify your strengths, weaknesses, and habits in presenting?      \\
To what extent did the full rehearsal practice page resemble an online presentation environment?             \\
How useful was the platform for practicing online presentations?  \\ \bottomrule
\end{tabular}%
}
\caption{7-scale Likert scale and open-ended questions asked to students in the post-survey.}
\label{tab:post-survey_questions}
\end{table*}
